Self-Confidence of Undergraduate Students in Designing Software Architecture

Software architecture students, often, lack self-confidence in their ability to use their knowledge to design software architectures. This paper investigates the relations between undergraduate software architecture students' self-confidence and their course expectations, cognitive levels, preferred learning methods, and critical thinking. We developed a questionnaire with open-ended questions to assess the self-confidence levels and related factors, which was taken by one-hundred ten students in two semesters. The students answers were coded and analyzed afterward. We found that self-confidence is weakly associated with the students' critical thinking and independent from their cognitive levels, preferred learning methods, and expectations from the course. The results suggest that to improve the self-confidence of the students, the instructors should work on improving the students' critical thinking capabilities.

==> data.tex <==
Perception [3, 3, 4, 6, 6, 2, 1, 1, 1, 3, 7, 7, 1, 3, 3, 3, 3, 3, 8, 5, 4, 2, 1, 1, 1, 4, 4, 7, 2, 1, 1, 5, 5, 16, 16, 5, 5, 1, 1, 1, 2, 4, 4, 12, 1, 1, 1, 1, 1, 2, 13, 2, 6, 9, 5, 2, 2, 1, 1, 10, 10, 1, 1, 1, 2, 2, 1, 2, 5, 3, 2, 5, 8, 1, 11, 1, 1, 1, 1, 2, 2, 10, 4, 1, 2, 9, 1, 14, 14, 15, 2, 1, 2, 2, 7, 7, 7, 7, 7, 2, 2, 2, 2, 2, 9, 9, 1, 1, 9, 2, 6, 14, 2, 2, 2, 2, 9, 2, 6, 2, 6, 6, 14, 14, 7, 7, 7, 7, 2, 1, 5, 14, 14, 1, 9, 14, 1, 1, 7, 2, 16, 16, 5, 2, 2, 7, 14, 2, 13, 13, 13, 14, 7, 1, 16, 14, 7, 7, 7, 7, 7, 9, 5, 14, 14, 2, 14, 14, 14, 16, 5, 5, 4, 7, 7, 7]
index [1, 2, 2, 3, 3, 4, 5, 5, 5, 6, 7, 7, 8, 9, 9, 10, 10, 10, 10, 11, 12, 13, 14, 14, 15, 16, 17, 17, 18, 19, 19, 20, 20, 21, 21, 22, 22, 23, 23, 24, 25, 26, 26, 27, 28, 28, 28, 29, 29, 30, 30, 31, 31, 32, 32, 33, 33, 34, 34, 35, 35, 36, 36, 36, 37, 37, 38, 39, 39, 40, 41, 41, 42, 43, 44, 45, 45, 46, 46, 47, 47, 48, 49, 50, 51, 51, 52, 53, 53, 54, 55, 56, 57, 58, 59, 59, 59, 60, 60, 61, 61, 62, 63, 64, 65, 65, 66, 66, 67, 68, 69, 69, 70, 71, 72, 72, 73, 73, 74, 75, 76, 76, 77, 77, 78, 78, 78, 78, 79, 80, 81, 82, 82, 83, 84, 84, 85, 85, 86, 87, 88, 88, 89, 89, 90, 91, 91, 92, 93, 93, 94, 94, 95, 96, 97, 98, 98, 99, 100, 100, 100, 101, 101, 102, 102, 103, 104, 104, 105, 106, 107, 107, 108, 109, 109, 110]
Cognitivelevel [4, 7, 7, 5, 5, 5, 2, 2, 2, 7, 2, 2, 2, 5, 5, 4, 4, 4, 4, 7, 5, 5, 5, 5, 5, 5, 4, 4, 4, 1, 1, 4, 4, 5, 5, 4, 4, 4, 4, 4, 6, 4, 4, 4, 4, 4, 4, 5, 5, 4, 4, 5, 5, 7, 7, 4, 4, 2, 2, 4, 4, 4, 4, 4, 4, 4, 4, 4, 4, 5, 5, 5, 5, 5, 2, 5, 5, 4, 4, 4, 4, 4, 4, 3, 4, 4, 5, 4, 4, 5, 7, 5, 4, 7, 2, 2, 2, 7, 7, 3, 3, 7, 4, 2, 5, 5, 4, 4, 5, 4, 7, 7, 7, 5, 4, 4, 4, 4, 4, 5, 7, 7, 4, 4, 5, 5, 5, 5, 7, 4, 2, 4, 4, 5, 4, 4, 4, 4, 5, 4, 4, 4, 5, 5, 7, 4, 4, 4, 4, 4, 7, 7, 5, 5, 5, 4, 4, 7, 4, 4, 4, 4, 4, 4, 4, 5, 4, 4, 4, 4, 5, 5, 4, 4, 4, 7]
Confidence [4, 2, 2, 2, 2, 4, 3, 3, 3, 5, 3, 3, 5, 1, 1, 1, 1, 1, 1, 4, 2, 2, 1, 1, 3, 3, 2, 2, 3, 2, 2, 2, 2, 1, 1, 3, 3, 1, 1, 1, 3, 3, 3, 1, 2, 2, 2, 2, 2, 2, 2, 2, 2, 5, 5, 5, 5, 4, 4, 5, 5, 4, 4, 4, 2, 2, 1, 3, 3, 1, 2, 2, 2, 5, 5, 1, 1, 3, 3, 3, 3, 2, 1, 1, 2, 2, 2, 1, 1, 1, 3, 2, 3, 2, 2, 2, 2, 2, 2, 1, 1, 2, 2, 4, 1, 1, 4, 4, 3, 1, 3, 3, 1, 1, 1, 1, 3, 3, 3, 2, 3, 3, 2, 2, 2, 2, 2, 2, 2, 2, 1, 1, 1, 1, 4, 4, 2, 2, 1, 3, 2, 2, 1, 1, 1, 1, 1, 1, 2, 2, 1, 1, 3, 3, 3, 3, 3, 1, 3, 3, 3, 2, 2, 2, 2, 1, 5, 5, 1, 2, 3, 3, 3, 1, 1, 1]
IOT_WEB [7, 3, 3, 2, 3, 4, 2, 3, 4, 4, 4, 1, 5, 1, 2, 2, 2, 2, 2, 3, 2, 3, 1, 1, 7, 2, 2, 3, 7, 1, 5, 2, 3, 2, 2, 1, 2, 2, 2, 1, 3, 3, 1, 1, 3, 3, 3, 2, 5, 1, 1, 1, 1, 7, 7, 5, 1, 5, 5, 2, 2, 2, 2, 2, 2, 2, 3, 1, 1, 2, 2, 2, 2, 7, 2, 1, 3, 3, 3, 3, 1, 1, 2, 1, 2, 2, 3, 5, 5, 1, 7, 7, 7, 2, 1, 2, 2, 2, 2, 2, 2, 7, 2, 7, 1, 1, 1, 1, 1, 1, 1, 3, 1, 3, 5, 5, 3, 3, 1, 7, 7, 7, 1, 3, 3, 3, 2, 1, 4, 2, 2, 1, 1, 5, 1, 5, 3, 5, 3, 3, 7, 7, 6, 6, 7, 1, 1, 1, 1, 3, 7, 7, 7, 7, 4, 3, 3, 7, 5, 5, 5, 7, 7, 2, 3, 3, 2, 3, 2, 3, 7, 7, 2, 2, 3, 1]
learnMethod [6, 4, 4, 3, 3, 12, 13, 13, 13, 7, 7, 7, 2, 8, 8, 1, 2, 4, 9, 1, 13, 4, 1, 2, 6, 1, 4, 4, 2, 1, 2, 8, 8, 7, 5, 5, 4, 8, 5, 3, 6, 1, 1, 4, 4, 14, 9, 5, 5, 3, 3, 6, 6, 8, 8, 3, 3, 1, 2, 3, 15, 1, 2, 3, 3, 13, 5, 2, 2, 6, 3, 3, 6, 10, 3, 3, 3, 4, 10, 5, 5, 4, 13, 6, 6, 6, 6, 2, 4, 10, 4, 1, 6, 13, 3, 8, 2, 3, 13, 2, 1, 3, 3, 10, 2, 8, 5, 11, 13, 4, 8, 8, 16, 13, 1, 5, 8, 8, 9, 6, 1, 2, 1, 2, 2, 1, 15, 7, 10, 13, 6, 4, 5, 6, 13, 13, 5, 5, 6, 3, 4, 11, 13, 13, 6, 3, 13, 13, 13, 13, 6, 6, 9, 6, 10, 13, 13, 8, 8, 14, 9, 8, 8, 1, 13, 7, 4, 13, 6, 13, 4, 5, 13, 8, 13, 13]
Effectiveness [2, 3, 3, 1, 1, 3, 4, 4, 4, 2, 2, 2, 2, 1, 1, 1, 1, 1, 1, 4, 1, 2, 1, 1, 3, 2, 2, 2, 1, 1, 1, 2, 2, 1, 1, 2, 2, 2, 2, 1, 4, 2, 2, 3, 2, 2, 2, 2, 2, 2, 2, 3, 3, 3, 3, 1, 1, 3, 3, 3, 3, 4, 4, 4, 3, 3, 1, 4, 4, 3, 2, 2, 4, 3, 3, 4, 4, 4, 4, 2, 2, 2, 4, 1, 4, 4, 2, 1, 1, 2, 3, 1, 4, 3, 2, 2, 2, 2, 2, 2, 2, 3, 2, 3, 2, 2, 2, 2, 4, 1, 1, 1, 1, 1, 1, 1, 3, 3, 2, 3, 3, 3, 3, 3, 2, 2, 2, 2, 2, 2, 2, 1, 1, 3, 3, 3, 1, 1, 2, 2, 2, 2, 3, 3, 4, 2, 4, 4, 4, 4, 3, 3, 3, 3, 3, 4, 4, 1, 2, 2, 2, 3, 3, 2, 2, 3, 2, 2, 3, 1, 4, 4, 2, 1, 1, 2]
group perception  Counter({1: 38, 2: 36, 7: 23, 14: 16, 5: 13, 3: 9, 4: 8, 9: 8, 6: 7, 16: 6, 13: 4, 10: 3, 8: 2, 11: 1, 12: 1, 15: 1})
group Cognitivelevel Counter({4: 88, 5: 46, 7: 22, 2: 14, 3: 3, 1: 2, 6: 1})
group Confidence Counter({2: 59, 1: 51, 3: 41, 4: 13, 5: 12})
group IOT_WEB Counter({2: 48, 1: 41, 3: 37, 7: 26, 5: 16, 4: 6, 6: 2})
group learnMethod Counter({13: 27, 3: 21, 6: 21, 4: 18, 8: 18, 1: 16, 2: 16, 5: 14, 7: 6, 10: 6, 9: 5, 11: 2, 14: 2, 15: 2, 12: 1, 16: 1})
corrCognitivelevelConfidence
[[ 0.  2.  0.  0.  0.]
 [ 1.  3.  5.  3.  2.]
 [ 3.  0.  0.  0.  0.]
 [23. 29. 22.  8.  6.]
 [18. 18.  8.  1.  1.]
 [ 0.  0.  1.  0.  0.]
 [ 6.  7.  5.  1.  3.]]
dependecy test for corrCognitivelevelConfidence
31.732763184814246 0.13375912239617097 24 36.41502850180731
p-value=0.133759, significance=0.05

At 0.05 level of significance, we accept the null hypotheses. 
	They are independent.
count 176
corrLearnMethodConfidence
[[ 4.  5.  4.  3.  0.]
 [ 5.  4.  4.  2.  1.]
 [ 4. 11.  1.  1.  4.]
 [ 5.  8.  4.  0.  1.]
 [ 5.  4.  4.  1.  0.]
 [ 9.  7.  4.  1.  0.]
 [ 2.  1.  2.  0.  1.]
 [ 6.  5.  5.  0.  2.]
 [ 1.  1.  3.  0.  0.]
 [ 1.  1.  2.  1.  1.]
 [ 0.  1.  0.  1.  0.]
 [ 0.  0.  0.  1.  0.]
 [ 8.  9.  7.  2.  1.]
 [ 0.  1.  1.  0.  0.]
 [ 0.  1.  0.  0.  1.]
 [ 1.  0.  0.  0.  0.]]
dependecy test for corrLearnMethodConfidence
63.69217871812162 0.3479083439235421 60 79.08194448784874
p-value=0.347908, significance=0.05

At 0.05 level of significance, we accept the null hypotheses. 
	They are independent.
count 176
corrIOTWEBCognitivelevel
[[ 1.  2.  1. 23. 11.  0.  3.]
 [ 0.  5.  2. 26. 12.  0.  3.]
 [ 0.  1.  0. 22.  9.  1.  4.]
 [ 0.  2.  0.  0.  2.  0.  2.]
 [ 1.  3.  0. 10.  2.  0.  0.]
 [ 0.  0.  0.  0.  2.  0.  0.]
 [ 0.  1.  0.  7.  8.  0. 10.]]
dependecy test for corrIOTWEBCognitivelevel
57.71709789101094 0.0122636587292944 36 50.99846016571065
p-value=0.012264, significance=0.05

At 0.05 level of significance, we reject the null hypotheses and accept H1. 
		They are not independent.
count 176
corrIOTWEBConfidence
[[18. 10.  9.  3.  1.]
 [16. 21.  4.  3.  4.]
 [ 6. 17. 12.  1.  1.]
 [ 0.  1.  3.  1.  1.]
 [ 5.  3.  3.  3.  2.]
 [ 2.  0.  0.  0.  0.]
 [ 4.  7. 10.  2.  3.]]
dependecy test for corrIOTWEBConfidence
39.875600845363905 0.022053868455142095 24 36.41502850180731
p-value=0.022054, significance=0.05

At 0.05 level of significance, we reject the null hypotheses and accept H1. 
		They are not independent.
count 176
corrPerceptionConfidence
[[10. 12.  7.  7.  2.]
 [11. 12.  9.  2.  2.]
 [ 6.  1.  0.  1.  1.]
 [ 1.  3.  4.  0.  0.]
 [ 2.  4.  5.  1.  1.]
 [ 0.  3.  4.  0.  0.]
 [ 6. 10.  7.  0.  0.]
 [ 1.  1.  0.  0.  0.]
 [ 2.  2.  2.  1.  1.]
 [ 0.  1.  0.  0.  2.]
 [ 0.  0.  0.  0.  1.]
 [ 1.  0.  0.  0.  0.]
 [ 1.  3.  0.  0.  0.]
 [ 7.  4.  2.  1.  2.]
 [ 1.  0.  0.  0.  0.]
 [ 2.  3.  1.  0.  0.]]
dependecy test for corrPerceptionConfidence
79.63746302384048 0.04580245208289176 60 79.08194448784874
p-value=0.045802, significance=0.05

At 0.05 level of significance, we reject the null hypotheses and accept H1. 
		They are not independent.


==> old Sections/Conclusion.tex <==

The study, reported in this paper, analyzed the relationships between students' confidence levels and their expectations, preferred learning methods, cognitive levels, and ability to synthesis knowledge.  The study found that the students confidence levels depends on their expectations from the course and their capabilities to synthesise the acquired knowledge but did not find dependency relationships between the confidence levels of the students and their cognitive levels or preferred learning methods. The results provide insight on the factors that make the students have better confidence in their abilities to design software architecture. Confidence in software architecture is required to be able to lead projects.

%Preferred learning methods and students expectations from the course are linked to students mindsets. for instance, a growing mindset students prefer active learning through e.g., practice exercise while fixed mindset students prefer passive learning methods. We plan to work on the relation of students mindset and their confidences and explore ways to change their mindsets and preferences to achieve better confidence. 







==> old Sections/Datacollection.tex <==
This section provides a summary of the responses of the students to the questionnaire and discusses the results.

\subsection{Confidence}

 

\begin{table}[bt]
\centering
\caption{Confidence of the students in their architecture designs.}
\label{tab:Confidence}
\rowcolors{2}{white}{lightgray}
%\renewcommand{\cellalign}{l}
\begin{tabular}{p{0.05in} p{0.5in} p{1.9 in} p{0.3 in} }
\hline
\rowcolor{Gray}\hline
 ID& Level	& Codes & \#Stu-dents\\\hline

1 & Confident & very confident, confident, pretty confident &	34 \\\hline

2 & Moderate confidence & somewhat confident, moderate, decent, somewhat confident, relative, quite confident &	34\\\hline

3 & Fair confidence & fair confidence, not very/extreme-ly/overly confident & 26\\\hline

 4 & No confident &not confident, not great  & 8\\\hline


 5 & No definite answer& no definite answer, no answer, not sure
 &	8\\\hline
\hline
\end{tabular}
\vspace{-0.2in}
\end{table}

This subsection reports about the results of the analysis of the responses to the question: {\tt How much confident would you be about your design?} We classified the extracted code into five categories: high confidence, moderate confidence, fair confidence, no confidence, and no definite answer. Table~\ref{tab:Confidence} shows the distribution of the confidence of the students. We observe that the number of students who believe that they gained confidence in designing software architecture is 31\%. We believe that these students gained confidence because they are comfortable with applying proven processes, such as \ac{ADD}. For instance, student {\tt(P24)} expressed that by saying that \emph{"I feel I would be very confident in my design, because I think the design process does a good job of ensuring the architecture considers and satisfies all the drivers. So as long as I am successful in compiling a thorough list of drivers, I think the design will turn out well."}. We found that 55\% of the students believe that they gained fair confidence in designing software architecture or better. Some of these students expressed the need to gain experience in industrial contexts to have better confidence in their architecture design. For instance, student {\tt(P7)} said: \emph{"I'm fairly confident in designing basic software applications, however I would still need some industry experience to become really confident in my abilities.}. Out of the remaining students, eight students (7\%) were not confident about their abilities to design architectures and eight students (about 7\%) did not provide definitive answers. Students who elaborated their answers expressed their need for a reference they could use to ensure efficacy of the architecture that they design. For instance, student {\tt(P32)} said \emph{"I don't really know, for everything we covered there were a lot of different views, but we didn't really know which one the best was. And a thing that bothers me a lot is how can we know that the QAs [Quality attributes] are addressed ? Ok I created an architecture, but I still don't know if the response time is less than 1 second or not. We have not done any testing, any coding..."}


\subsection{Student' expectations about the course}

\begin{table}[bt]
\caption{Student's expectations about the course.}
\label{tab:Perception}
\centering
\rowcolors{2}{white}{lightgray}
\renewcommand{\cellalign}{l}
\begin{tabular}{p{0.1in} p{2.2in} p{0.6 in} } 
\hline
\rowcolor{Gray}\hline
ID & Expectation & \#Students \\ \hline
1&No expectation &	23 \\\hline
2&Design of architecture &	26\\\hline
3&Curious about the topic	& 4 \\\hline
4&Relation to another course &	6\\\hline
5&Heavy coding &	9\\\hline
6&Types of architecture &	4 \\\hline
7&Architectures styles & 12\\\hline
8&Relate to internship & 2\\\hline
9&Design pattern  &	3\\\hline
10&Theoretical	& 2\\\hline
11&Group project class	& 1\\\hline
12&Software development &	1\\\hline
13&Architecture evaluation & 2\\\hline
14&	Design process&	10\\\hline
15&	Design practices& 1\\\hline
16&	Other&	4\\\hline\hline
\end{tabular}
\vspace{-0.2in}
\end{table}


The students have their own expectations form the course based on other courses, discussion with colleagues

This subsection reports about the results of the analysis of the replies to the question: {\tt What was your expectation of the course before taking it?} Table~\ref{tab:Perception} shows the expectations of the students about the course before taking it--reported at the end of each of the semesters.. 

In general, the students expected the course to be about design of architecture (23.6\%), architecture styles (10.9\%), or design process (9.1\%). In addition, we observe that six students related the course to other courses. For example, student {\tt(P16)} said \emph{"I thought that it would be similar to 319."} Moreover, we observe that two students had experience with architecture in their internships and related the course to that experience. For instance, {\tt(P42)} said \emph{"Initially I assumed the course would cover what effectively boils down to self-congratulatory discussion filled with buzz-words. The software architectures I have seen through working for software development companies are often a chaotic mess of anti-patterns and individuals attempting to defend decisions by calling them architectural drivers. Before the course even began this was what I expected to experience."} We also observe from Table~\ref{tab:Perception} that the percentage of students who did not have clear expectations about the course are 20.9\%. The reason of this high percentage is possibly due to the fact that the course is required for their program of study.

\subsection{Cognitive levels}

This subsection reports about the results of the analysis of the replies to the question: {\tt Assume you are given a project and asked to design an architecture for it. How would you do the design?} We coded the responses of the students. We classified the extracted codes based on the new Bloom taxonomy cognition levels~\cite{GaKAC2000}. Column 1 and 2 of Table~\ref{tab:BloomLeaning} show the classification of the codes to Boom's cognition categories. 

\begin{table}[bt]
\caption{Cognitive levels of the students.}
\label{tab:BloomLeaning}
\centering
\rowcolors{2}{white}{lightgray}
%\renewcommand{\cellalign}{l}
\begin{tabular}{p{0.05in} p{0.5in} p{1.9in} p{0.3 in} } 
\hline
\rowcolor{Gray}\hline
ID & Cognition category & Codes & \#Stu-dents\\ \hline
1 & Creating & adjust design process	& 1\\ \hline
2 & Evaluat-ing & identify trade-offs, identify risk, architecture evaluation	& 8\\ \hline
3 & Analyzing & analysis & 2\\ \hline
4 & Applying & identify architecture drivers, get requirements, meet stakeholders, create design, apply the design process, do as in assignments, modify reference architecture & 50\\ \hline
5 & Understa-nding & select reference architecture, select architecture style, select architecture type, make diagrams & 32\\ \hline
6 &  Rememb-ering	&	& 1\\ \hline
7 & Irrelevant	&	& 16 \\ \hline\hline

\end{tabular}
%\vspace{-0.1in}
\end{table}

We observe that most of the students have "applying" and "understanding" cognitive levels. We also observe that the number of students who provided irrelevant answers are sixteen (14.5\%). Many of the students specified that they need more details to decide how to proceed with the design or provided non-useful answers such as \emph{"I would probably try and lay out the entire system's architecture in one go because the process of iterations confused me."} {\tt(P11)}. In addition, we observe that few students had the "evaluating" cognitive level,  one student had the "creating" cognitive level, and one student had the "remembering" cognitive level.

\subsection{Preferred learning method}


This subsection reports about the results of the analysis of the replies to the question: {\tt What is/are the method(s) that helped you better learn software architecture?} Table~\ref{tab:lernmethod} reports about the frequencies of preferred learning methods reported by the students. Recall that each student can specify one or a set of preferred learning methods. 

\begin{table}[bt]
\caption{Students preference of the learning methods.}
\label{tab:lernmethod}
\centering
\begin{tabular}{p{0.1in}p{2.2in}p{0.6 in}} 
\hline
\rowcolor{Gray}\hline
ID &Learning method	& \#Students\\\hline
\rowcolor{lightgray}
1&Group assignments&	16\\\hline
2&Individual assignments&	16\\\hline
\rowcolor{lightgray}
3&Case studies&	21\\\hline
4&Reading&	18\\\hline
\rowcolor{lightgray}
5&In-class group activities&	14\\\hline
6&No definitive answer&	21\\\hline
7&Quizzes&	6\\\hline
\rowcolor{lightgray}
8&Drawing diagrams&	18\\\hline
9&	Evaluate work of peers&	5\\\hline
\rowcolor{lightgray}
10&Learning on own&	6\\\hline
11&Assignments &	2\\\hline
\rowcolor{lightgray}
12&Other courses &	1\\\hline
13&Practice&	27\\\hline
\rowcolor{lightgray}
14&In-class posters&	2\\\hline
15 & Lectures &	2\\\hline
\rowcolor{lightgray}
16&	Live demo&	1\\\hline
\hline
\end{tabular}
%\vspace{-0.2in}
\end{table}

We observe that the percentages of students who prefer passive learning methods (lecture, reading, and quizzes) are 14.8\%  and the percentage of students who prefer active learning methods such as assignments (group assignments and individual assignments, practice, in-class posters, in-class activities, and evaluating the work of peers) is about 45.5\%. (We excluded the methods that could be considered in both learning styles). 




\subsection{Capability to synthesise acquired knowledge}

\begin{table}[btp]
\caption{Capability to synthesise acquired knowledge.}
\label{tab:cabsynthesis}
\centering
\rowcolors{2}{white}{lightgray}
%\renewcommand{\cellalign}{l}
\begin{tabular}{p{0.06in} p{0.6in} p{1.8in} p{0.3in} } 
\hline
\rowcolor{Gray}

ID & Aspect & Codes &	\#Stu-dents\\\hline
		
1 & Architec-ture drivers &  reliability, interoperability, scalability, architecture drivers, availability, performance,and security requirements & 41\\ \hline
		
		
2 & Patterns of the structures of the solutions & communication pattern, components structure (e.g., modularity), control of physic, Objects vs logic computation, interacting actors, access to arch. components, flexibility to add components, integration of complex software &	48\\ \hline
		

3 & Architectural knowledge & Reference architecture, architecture styles, architecture patterns &	37\\ \hline

4 & Simplici-ty & simplicity and complexity &	6\\	 \hline


5 & Technolo-gy stack & technology stack, security protocols, use of hardware, complexity of software &	16	\\ \hline

6 & Configura-tion manage-ment & Configuration management &	2\\\hline

7 & No definite answer & &	26\\\hline\hline
\end{tabular}
%\vspace{-0.2in}
\end{table}

 This subsection reports about the results of the analysis of the replies to the question: {\tt What are the differences between designing the architecture of a Web application and the one of an IoT system?} Table~\ref{tab:cabsynthesis} summarizes the answers to the question above. The codes that we derived from the answers are classified into six categories. The first category, architecture drivers, includes codes that are related to requirements that are used in designing architectures, such as reliability and scalability. The second category, patterns of the structures of the solutions, includes codes such as communication patterns and whether the application is for controlling physical objects or performing logical computation. The third category, architectural knowledge, includes codes such as reference architecture and architecture patterns. The fourth category, simplicity, includes only code "simplicity." The fifth category, technology stack, includes codes, such as technology stack and security protocols. The sixth category, configuration management, which includes one code--configuration management--was reported by one student. Note that a student could identify differences in more than one category; that is, a student could discuss performance, which is an architecture driver, and distribution of the system's components, which we classify as patterns of the structures of the solutions.

We observe that the percentage of students that discussed architecture drivers are 23.3\%, architecture knowledge 21\%, and technology stacks 9.1\%. We observe also that the number of students who expressed that the two types of systems use different architecture structure patterns are the largest that is 48 (28.7\%). In addition, we observe that the number of students who did not provide definitive answers are 26 (23.6\%). Some of these 26 students reported that they do not know and the others did not answer the question or provided non-useful answers such as \emph{"I thought this was a survey, not a test."}


==> old Sections/Researchmethod.tex <==
We conducted a qualitative study to assess the factors affecting the confidence of the students in designing software architecture. The study uses students' responses to a questionnaire as data source. We discuss in the following the preparation of the study, the data collection, and the data analysis activities. 

%\todo[inline]{grades of the exams and assignments depend on the easiness of the questions/problems. We did not use them in the study.}

\vspace{.1in}
\noindent {\bf Preparation of the study.} We discussed the course with colleagues and identified a set of factors that could be used to evaluate the students confidence and course effectiveness, which are: (1) cognitive levels by the students, (2) preferred learning method, and (3) capability of the students to synthesis acquired knowledge. Therefore, we used expert opinions rather than literature review to identify the factors that may impact the confidence of the students in designing software architecture. The factors were used to develop a set of questions to measure them, which are listed in Table~\ref{tab:questionaire}. 

\begin{table}[tb]
\caption{Questionnaire.}
\label{tab:questionaire}
\centering
\begin{tabular}{p{0.1in}p{0.9in}p{1.9in} } 
\hline
\rowcolor{Gray}\hline
ID & Factor & Question\\ \hline
\rowcolor{lightgray}
1& Expectation & What was your expectation of the course before taking it?\\\hline
2& Cognitive level & Assume you are given a project and asked to design an architecture for it. How would you do the design?\\\hline
\rowcolor{lightgray}
3& Confidence to design architecture& How much confident would you be about your design?\\\hline
4& Capability to synthesis acquired knowledge & What are the differences between designing the architecture of a Web application and the one of an \ac{IoT} system?\\\hline
\rowcolor{lightgray}
5& Preferred learning method & What is/are the method(s) that helped you better learn software architecture? \\\hline\hline
\end{tabular}
\vspace{-0.2in}
\end{table}


We developed an anonymous, electronic questionnaire using Google Form and made it available online for the students in November 2017 (for Fall 2017 semester) and April 2018 (for Spring 2018 semester).\footnote{The project was granted an IRB exemption.} (The students answer the questionnaire at the  end of the semester.) The submissions were anonymous, but the students had to tell the instructor that they participated in the study to get their bonus points. 


\vspace{.1in}
\noindent {\bf Data collection.} One-hundred ten students answered the questionnaire in Fall 2017 and in Spring 2018. We read the answers and we used the thematic analysis~\cite{saldana2015coding} method to code all the questionnaire responses. A code is a word or short phrase identifying the essence of a portion of language-based or visual data. Coding uses the responses as input and outputs codes that identify the aspects mentioned in the responses~\cite{BrGr2007}. At the end of this step we assigned codes to each of the responses of the one-hundred ten students. Thus, we obtain a set of categories for each of the factors of Table~\ref{tab:questionaire}.

The cognitive levels according to Bloom taxonomy of the students ~\cite{GaKAC2000} are commonly assessed either using test questions or reflection write-ups~\cite{HBF2019}. We used in this study the verbalization\footnote{See for example: https://adp.uni.edu/documents/ bloomverbscognitiveaffectivepsychomotor.pdf} used by the students in their responses to reflection Question 2 to identify the cognitive level of each of the students. The association of the verbs to the different levels is based on the author' domain knowledge. For instance, Participant {\tt(P20)} said \emph{"The design would vary depending on what the project requirements and architectural drivers were. Once I decided on an optimal reference architecture, I would go through the iteration design process and make sure that appropriate design decisions were made to address every architectural driver that was identified in the project description."} The codes extracted from the statements are: "apply design process", "select reference architecture", and "evaluate." Since the code "evaluate" is classified in the cognitive levels as {\tt Evaluation}, we classified the student at level {\tt Evaluation}--that is, the code associated with the higher cognitive level is selected.

Next, we counted the frequency of the different codes used in the responses to each of the questions of Table~\ref{tab:questionaire} and observed the patterns in these data. We report the data that we collected in Section~\ref{sec:resultexplore}.

\vspace{.1in}
\noindent {\bf Data analysis.} We represented the relationships between the students' confidence and each of the factors affecting their confidence using matrices--we use one matrix for each factor. The columns of the matrix are the confidence levels, the rows are the codes of the factor being studied, and the elements are the frequencies of the students who belong to the given factor category and given confidence level. We use Chi-square independence test~\cite{Cochran1952} to evaluate the dependencies between the confidence level factors and the related factors. In addition, we used the heat map diagram to visualize these relationships. A heat map is a graphical representation of data where the individual values contained in a matrix are represented as colors. The colors range from brown, red, yellow, green, blue, to dark blue, where brown indicates the highest frequency and dark blue indicates zero.

In addition, we used the correlation technique to study the relationship between the confidence levels of the students and their perceptions of the effectiveness of the course. 


==> old Sections/abstract.tex <==




==> old Sections/coursedesign.tex <==
The course Software Architecture Design is an undergraduate level course for the software engineering and the computer engineering programs. Before taking the class, the students take a class on developing web applications. The course is given two times a year. Each semester, the class meets 2 times a week for 14 weeks, each of 75 minutes.
 
We discuss in the following the course objectives and structure.



\begin{table}[tb]
\caption{Modules for the software Architecture design course.}
\label{tab:modules}
\centering
\begin{tabular}{p{.1in} p{1.8in}  p{0.3 in} p{.5in} } 
\hline
\rowcolor{Gray}\hline
ID& Module & \# of sessions & Teach. form\\ \hline
\rowcolor{lightgray}
1 & Overview of software architecture& 2 & R, GA \\\hline
2 &\ac{UML}& 3 & R, GA, IA \\\hline
\rowcolor{lightgray}
3 & Architecture styles, patterns, and tactics& 4 & L, R, GA\\\hline

4 & Architecture drivers& 5 & R, PA, GA, IA\\\hline
\rowcolor{lightgray}
5 & Architecture design process&4& R, GA, PA, IA\\\hline

6 & Documenting a software architecture&1& R, GA \\\hline
\rowcolor{lightgray}
7 & Architecture evaluation& 2& R, GA, IA \\\hline

8 & Software security architecture&1& L\\\hline
\rowcolor{lightgray}
9 & Architecture recovery&1&L \\\hline\hline

\end{tabular}

\begin{flushleft}The notation is: Reading (R), Group Activities (GA), Lecture (L), Individual Assignments (IA), and Project Assignment (PA).\end{flushleft}

%\vspace{-0.3in}
\end{table}

\subsection{Course objectives}

The goal of the course is to train the students on designing software architecture. We choose to use the \acf{ADD} method, which applies a process-based approach to the design of software architecture~\cite{HKNO2005, CeKa2016}. Thus, to design an architecture, the students follow three major phases: eliciting architecture drivers, designing architecture that meets the drivers, and evaluating a given architecture. The main goals of the course are acquiring knowledge needed to design software architecture and learning how to perform the three phases described above. The objectives are:

\begin{enumerate}
\item understand what a software architecture is and explain why it is important,
\item understand the relationships between software quality attributes and software architecture,
\item ability to elicit software architecture drivers,
\item ability to use architecture styles, patterns, and tactics,
\item ability to use the attribute-driven method to design software architecture,
\item ability to document software architecture,
\item ability to evaluate software architecture.
\end{enumerate}

\subsection{Course structure}

The course objectives were refined to identify the course modules, listed in Table~\ref{tab:modules}. The table provides for each module the number of sessions and the teaching form.

\begin{table}[tb]
\caption{List of assignments.}
\label{tab:assignments}
\centering
\begin{tabular}{p{0.8in}  p{2.25 in} } 
\hline
\rowcolor{Gray}\hline
Type	& Description\\ \hline
\rowcolor{lightgray}
Individual assignment 1 &   Practice with UML diagrams.	\\\hline
Group assignment~1 &   Experiment with the identification of architectural drivers for a given project.\\\hline
\rowcolor{lightgray}
Group assignment~2&   Experiment with the design of an architecture for a given project.\\\hline
Individual assignment~2&  	Experiment with the design of an architecture for a given project.	\\\hline
\rowcolor{lightgray}
Individual assignment~3 &	Evaluate the architecture of a software	\\\hline
Group assignment~3 &	Implement a designed architecture and reflect about the gap between as-designed and as-implemented architecture.\\ \hline\hline
\end{tabular}
\vspace{-0.2in}
\end{table}

We applied in this course the Team-based learning method~\cite{SORM2014}. The students were given book chapters and papers, selected from~\cite{CeKa2016,Gor2006,Fow2000,Ebe2017}, to {\tt read} before coming to class. The students take an online quiz to test their readiness to discuss the topic. The quiz questions are  discussed afterwards in-class. As exception, modules eight and nine were designed as lectures because they are considered as complementary.

Next, the students work in groups on in-class activities. The activities include answering questions that need reflection, working on exercises, and simulating architecture meetings. In these activities, all the groups provide their answers at the same time. They are asked afterwards to justify their answers and discuss them with their colleagues and instructor. The case studies provided by ~\cite{CeKa2016} were very useful for the students to see how the techniques could be used.

The students were requested to practice with their knowledge in a set of assignments, described in Table~\ref{tab:assignments}, in the order they are given to the students. The group assignments consist of extending an existing software,\footnote{It was developed in a previous class by a team of students.} given to the students. The students work in groups on the project in three group assignments: gathering architectural drivers, designing the architecture of the new version of the software, and implement the architecture they designed. The individual assignments enforce the experience that the students obtained from the project. The assignments cover gathering architectural drivers for a given project, design a solution that addresses a set of given architecture drivers, and evaluate the architecture design of a colleague. The group assignments are related to an \ac{IoT} project, while the individual assignments are related to IT projects. This should give the students an experience with the two domains. 

In addition, few sessions were dedicated to extra activities: visit of professionals, panel that includes a representative of each team, and a research talk by the instructor. First, the students benefit from the visit of a software architect from a big local organization. The visitor gives a presentation about their architecture problems, the designs they adopted, and the struggle they live-in to continuously provide better products. The students are expected to link the principals, techniques, and activities they practice with in-class to the professional practice of the architecture design. Second, the different teams faced different architectural challenges when working on their projects. Representatives of the teams form a panel and take turn in answering questions from the instructor and the students. The questions are designed to make the panelists reflect about their experience and share the experience they acquired in working on their respective projects. Third, the instructor gives a talk on a recent research topic related to the course. The goal is to encourage the students to appreciate scientific research.


==> old Sections/dataanalysis.tex <==
We analyze in this section the relationships between students' confidence levels to design architecture by the end of both semesters and the students' expectations, their ability to synthesis acquired knowledge, their cognitive levels, and their preferred learning method. We use in this analysis the Chi-square independence test~\cite{Cochran1952} with 90\% confidence and the heat map techniques discussed in Section~\ref{sec:resmethod}. 

\subsection{Students' expectations.}

\begin{figure}
   %\vspace{-1.0in}
    \centering
{\includegraphics[width=0.5\textwidth, keepaspectratio]{Figures/fig/expectationConfidence.png}}
  \caption{Relationship between expectations and confidence levels. See Table~\ref{tab:Confidence} for the confidence levels and Table~\ref{tab:Perception} for the expectation categories. The colors range from brown, red, yellow, green, blue, to dark blue, where brown indicates the highest frequency and dark blue indicates zero.}
\label{fig:PerceptConfidence}
%\vspace{-0.2in}
\end{figure}

The Chi-square test of dependence confirms the dependency between the students' confidence levels and their expectations, with $\chi^2$ of 79.6 and p-value 0.04. A more detailed analysis follows. Figure~\ref{fig:PerceptConfidence} shows the heat map diagram for the expectation vs. confidence of the students. First, we observe that the students who have no expectations are mostly either confident (10 students) or have moderately confidence (12 students) in their ability to design architecture. We observe that the students with high confidence in their abilities to design confidence have expectation that the course about design of architecture (11 students), the design process (7 students),architecture styles (6 students), and curios about the topic (6 students). We observe, in addition that the students have moderate confidence in their ability to design architecture expected the course to about the design of architecture (12 students), and architecture styles (10 students). These results suggest that the students who have no expectation or correct expectation achieve better confidence in their ability to design architecture. This result suggests that the instructor should ensure that the students have correct expectations from the course. 
%done

\begin{figure}
  % \vspace{-1.0 in}
    \centering
{\includegraphics[width=0.4\textwidth, keepaspectratio]{Figures/fig/cognitiveConfidence.png}}
  \caption{Relationship between cognitive levels and confidence levels. See Table~\ref{tab:BloomLeaning} for the cognitive levels and Table~\ref{tab:Confidence} for the confidence categories. The colors range from brown, red, yellow, green, blue, to dark blue, where brown indicates the highest frequency and dark blue indicates zero.}
\label{fig:CognitiveConfidence}
%\vspace{-0.2in}
\end{figure}

\subsection{Capability to synthesise acquired knowledge.}

The Chi-square test of dependence confirms the dependency between the students' confidence levels and their capability to synthesise acquired knowledge, with $\chi^2$ of 39.87 the p-value is 0.022. A more detailed analysis follows. Figure~\ref{fig:WebIOTConfidence} shows the heat map diagram for the ability of the students to differentiate IOT-based and Web-based architectures vs. their confidence in designing software architecture. The figure shows that the students who have good confidence in their ability to design software architecture discuss more the difference in the architecture drivers and the difference in the patterns of the structures of the solutions and to lesser frequency the architecture knowledge. We observe also that the students who have moderate confidence discuss more the differences in the patterns of the structure of the solutions and the architecture knowledge and to lesser frequency the differences in the architecture drivers between the two software types. In addition, we observe that the students who did not show their abilities to differentiate between IOT-based and Web-based architecture have mostly fair confidence. We note that the students who have good, moderate, and fair confidence are mostly able to identify differences in the architecture drivers, patterns of the structures of the solutions, and architecture knowledge between the two software types . 
 %doone
 \begin{figure}
   %\vspace{-1.0in}
    \centering
    {\includegraphics[width=0.4\textwidth, keepaspectratio]{Figures/fig/learnConfidence.png}}
        %\caption{Fall 2017}
    \caption{Relationship between preferred learning methods and confidence levels. See Table~\ref{tab:Confidence} for the confidence levels and Table~\ref{tab:lernmethod} for the preferred learning methods.}
    \label{fig:learningmethodconfidence}
 %   \vspace{-0.2in}
\end{figure}

\subsection{Student' cognitive levels.}

The Chi-square test of dependency confirms the independence between the students' cognitive levels and their confidence level with 90\% confidence, $\chi^2$ of 21.95 and p-value of 0.58. A more detailed analysis follows. Figure~\ref{fig:CognitiveConfidence} shows the heat map diagram for the cognitive levels of the students vs. their confidence in designing software architecture. We observe that the students who have applying cognitive level do not necessarily have good confidence--14 students have good confidence, 16 students have moderately confidence, and 13 students have fair confidence in their ability to design architecture. We observe also that the students who have understanding cognitive level do not necessarily have fair confidence--12 students have good confident level, 11 students have moderate confidence, and 7 students have fair confidence on their ability to design architecture. We observe, however,that the students who have creating and evaluating cognitive level have moderate, fair or no confidence. The paradox of low-performers exhibiting high confidence and high performers exhibit under-confidence is documented in other domains such as accounting ~\cite{RWW2012}. A possible reason is that the high performers know the limit of their abilities.  

Note that, the students who did not provide enough information to identify their cognitive levels have mostly good and moderate confidence levels. We looked at the responses of these students and we observe that they asked for more details to be able to answer the question related to the cognitive levels.

The results of the relationship between the cognitive levels and the confidence levels of the students are counter intuitive. They suggest that cognitive levels do not discriminate the confidence levels of the students. 
%done
\begin{figure}
 %  \vspace{-1.0in}
    \centering
    {\includegraphics[width=0.4\textwidth, keepaspectratio]{Figures/fig/iotwebConfidence.png}}
    \caption{Relationship between the ability of the students to synthesis knowledge and confidence levels. See Table~\ref{tab:Confidence} for the confidence levels and Table~\ref{tab:cabsynthesis} for aspects that the students identify when differentiating the architectures of Web applications and IOT-based software.}
    \label{fig:WebIOTConfidence}
    %\vspace{-0.2in}
\end{figure}

\subsection{Students' preferred learning methods.}

The Chi-square test of dependency confirms the independence between the students' confidence levels and their learning method with 90\% confidence, $\chi^2$ of 63.69 and p-value of 0,34. A more detailed analysis follows. Figure~\ref{fig:learningmethodconfidence} shows the heat map diagram for the students' preferred learning methods vs. their confidence levels in designing software architecture. We observe that the students who prefer to learn from case studies have mostly moderate confidence level (11 out of 21) and the students who prefer practice as a learning methods have mostly good, moderate, or fair confidence levels (24 out of 27 students). We also observe that the students who prefer reading have mixed confidence levels (5 have good confidence, 8 have moderate confidence, and 4 have fair confidence). In addition, we observe that the students who did not provide a definitive answer to the preferred learning method question have mostly good or moderate confidence (9 and 7 respectively out of 21 students).  The results suggest that providing the students with practice opportunities helps them to gain better confidence.

We did not see major patterns from the analysis of the students who expressed that they would not be confident about their design. We found that these students have varying preferred learning methods (including practice), varying expectations from the class, and different cognitive levels. 
%done

 \begin{figure}
 
    \centering
    {\includegraphics[width=0.4\textwidth, keepaspectratio]{Figures/fig/iotwebCognitive.png}}
        %\caption{Fall 2017}
    \caption{Relationship between ability to synthesis knowledge and cognitive level. See Table~\ref{tab:Confidence} for the confidence levels and and Table~\ref{tab:BloomLeaning} for the cognitive levels.}
    \label{fig:WebIOTCognitivelevel}
 %   \vspace{-0.2in}
\end{figure}

==> old Sections/introduction.tex <==



==> old Sections/limitations.tex <==

\subsection{Impacts of the study}

This article reports about an exploration of the factors that impact the confidence of undergraduate students in their abilities to design architecture after taking a course on software architecture. The study found that the students confidence levels depends on their expectations from the course and their capabilities to synthesise the acquired knowledge. It did not find, however, dependency relationships between the confidence levels of the students and their cognitive levels or preferred learning methods. Thus, the students ability to design software architecture when they graduate does not depend on their expressed cognitive levels--and potentially their score in the class.\footnote{We cannot correlate the data with the students assessment scores in the class because we did not request that in the  IRB before starting the study.} The results suggest that the instructors should ensure that the expectations of the students are aligned with the course goals and try to use case studies that shows contrasts, e.g., performance needs for Web applications and IOT-based software.

The study focuses on the relationships between education factors (e.g., capabilities to synthesis acquired knowledge) and confidence of the students. The results show that the better the students are able to synthesise knowledge, the better they are confident in their abilities to design architecture. The proverb "if all you have is a hammer, everything looks like a nail" seems to apply to designing architecture for undergraduate students. This suggests that instructors should teach the students some knowledge about \emph{alternative solutions} for solving given architecture problems, so they understand that there are conditions and implications of using architecture knowledge to solve architecture problems, before asking them to apply architecture design methods~\cite{HOFMEISTER2007106}. 

\subsection{Limitations of the study}

The main limitations of the study follow. First, We did not find studies on the confidence of undergraduate students to design software architecture. Colleagues may argue in private that it is difficult to measure the students' perceptions of their confidences. We agree with the assessment and we hope the work helps to initiate the discussion about measuring the construct of self-confidence of students--given that this trait is very important for students to take initiatives. 

Second, we did not use a repeatable process to identify the factors that affect the confidence levels of the students; we selected them in brainstorming sessions with colleagues: there may be other factors that impact the students' confidence, but these were judged to be relevant to the instructors. Second, 

Third, the students provided their responses in text and the author and a teaching assistant coded the responses. The codes were used to associate students with levels or categories of the factors. We acknowledge that the perspective of the response coders may have impacted the data extraction. We, however, revisited the data extraction several times to reduce this limitations. We also cross-checked often the students' answers. We used, for instance, Figure~\ref{fig:WebIOTCognitivelevel} which describes the relationships between the ability of the students to synthesis knowledge and their cognitive levels. The figure shows that some of the students (10 out of 16) are not associated with specific cognitive levels but provided differences between IOT-based and Web-based architectures, which leads us to double-check our coding.

The study was performed in two semesters in raw with only minor change to the content--we added one lecture on architecture styles in Spring 2018. The number of students for both semesters one-hundred ten--all are junior or senior undergraduate students. The study, however, was carried out in only one university, which may limit the generalization of the results.







%\todo[inline]{Students who provided irrelevant answers for cognitive levels provided also irrelevant answers for differentiating IOT-based and Web-based architecture}

